Sized Types with Usages for Parallel Complexity of Pi-Calculus Processes

We address the problem of analysing the complexity of concurrent programs written in Pi-calculus. We are interested in parallel complexity, or span, understood as the execution time in a model with maximal parallelism. A type system for parallel complexity has been recently proposed by Baillot and Ghyselen but it is too imprecise for non-linear channels and cannot analyse some concurrent processes. Aiming for a more precise analysis, we design a type system which builds on the concepts of sized types and usages. The new variant of usages we define accounts for the various ways a channel is employed and relies on time annotations to track under which conditions processes can synchronize. We prove that a type derivation for a process provides an upper bound on its parallel complexity.

==> altrules.tex <==
\begin{figure*}
	\centering
	\begin{framed}
		\begin{center}
			%Channel Input  			
			\AXC{$\fifi;\Gamma, a \COL \ChT{\seq{T}}{U}, \seq{\var} \COL \seq{T} \p P \C K$}
			\UIC{$\fifi;\Up{J_c}{\Gamma}, a \COL \ChT{\seq{T}}{\IU{[0,0]}{J_c}.U} \p \In{a}{\seq{\var}}.P \C J_c;K$}
			\DP 
			\qquad
			%Channel Output 
			\AXC{$\fifi;\Gamma', a \COL \ChT{\seq{T}}{V}  \p \seq{e} \COL \seq{T} \qquad \fifi;\Gamma, a \COL \ChT{\seq{T}}{U} \p P \C K$}
			\UIC{$\fifi;\Up{J_c}{(\Gamma \PAR \Gamma')}, a \COL \ChT{\seq{T}}{\OU{[0,0]}{J_c}.(V \PAR U)} \p \Out{a}{\seq{e}}.P \C J_c;K$}
			\DP 
			\\ 
			\vvskip 
			%Server Output
			\AXC{$\fifi;\Gamma', a \COL \ServT{\seq{i}}{K}{\seq{T}}{V}  \p \seq{e} \COL \Isub{\seq{T}}{\seq{i}}{\seq{\INN{I}}} \qquad \fifi;\Gamma, a \COL \ServT{\seq{i}}{K}{\seq{T}}{U} \p P \C K' $}
			\UIC{$\fifi;\Up{J_c}{(\Gamma \PAR \Gamma')}, a \COL \ServT{\seq{i}}{K}{\seq{T}}{\OU{[0,0]}{J_c}.(V \PAR U)} \p \Out{a}{\seq{e}}.P \C J_c;(K' \cup \Isub{K}{\seq{i}}{\seq{\INN{I}}})$}
			\DP 
		\end{center}
                \(J_c;K\) is defined as follows.
                \[
                  [I,J];[K_1,K_2] = \left\{\begin{array}{ll}
                    [0,0] &\mbox{if $I= \infty$}\\{}
                    [0,J+K_2] &\mbox{otherwise}\\
                  \end{array}\right.
                  \]
                  \NK{Intuition: \(J_c;K\) represents the complexity of an input/output process
                    when the input/output has capacity \(J_c\) and
                    the complexity of the continuation is \(K\).
                     \(J_c=[\infty,\infty]\) means the input/output will never
                     succeed (because there is no corresponding output/input); hence
                     the complexity is \(0\). Otherwise, an upper-bound is given by
                     \(J+K_2\) (the time spent for the input/output to succeed, plus \(K\)).
                     The lower-bound is \(0\), since the input/output may be blocked forever.
                    }
	\end{framed}
	\caption{Alternative Typing Rules for Processes with Usages}
	\label{f:usagetype:alt}
\end{figure*}

